Shedding light on Dark Matter through 21 cm Cosmology and Reionization constraints

During the last decades, our understanding of the universe has reached a remarkable level, being able to test cosmological predictions with an astonishing precision. Nonetheless, the nature, composition, mass and interactions of the Dark Matter still remain unknown, presenting one of the most intriguing conundrums in current cosmology. In this doctoral thesis, signatures of Dark Matter candidates which can leave an impact on the process of formation of structures and on the evolution of the Intergalactic Medium are studied. This thesis is organized in three parts. Part I is devoted to a broad introduction to the fundamentals, describing the state of the art of the topics considered. The basics of the $\Lambda$CDM are presented in Chapter 1. Chapter 2 overviews the historical progress of evidences of Dark Matter, followed by a discussion of the status and small-scale issues of the Cold Dark Matter paradigm, examining two alternative non-standard scenarios: Warm Dark Matter and Interacting Dark Matter. Chapter 3 considers Primordial Black Holes as another Dark Matter candidate, discussing the effects of accretion of surrounding matter and the enhancement of small-scale fluctuations due to the Poisson shot noise, both of which could leave an observational impact in the Intergalactic Medium. The fundamentals of the 21 cm cosmological signal are reviewed in Chapter 4, summarizing the main processes which drive the brightness temperature, and discussing its spatial fluctuations via the power spectrum. Finally, Chapter 5 is dedicated to the ionization and thermal evolution of the Intergalactic Medium during the Cosmic Dawn and the Reionization epochs. Part II includes seven original scientific articles published during the development of the PhD, which constitute the main work of this thesis. Finally, Part III contains a summary of the main results in Spanish.

==> Chapters/Others/Acknowledgements_pre.tex <==

\chapter*{Agradecimientos}
\addcontentsline{toc}{chapter}{Agradecimientos}  

Blablabla












